Scalable Machine Learning Training Infrastructure for Online Ads Recommendation and Auction Scoring Modeling at Google

Large-scale Ads recommendation and auction scoring models at Google scale demand immense computational resources. While specialized hardware like TPUs have improved linear algebra computations, bottlenecks persist in large-scale systems. This paper proposes solutions for three critical challenges that must be addressed for efficient end-to-end execution in a widely used production infrastructure: (1) Input Generation and Ingestion Pipeline: Efficiently transforming raw features (e.g., "search query") into numerical inputs and streaming them to TPUs; (2) Large Embedding Tables: Optimizing conversion of sparse features into dense floating-point vectors for neural network consumption; (3) Interruptions and Error Handling: Minimizing resource wastage in large-scale shared datacenters. To tackle these challenges, we propose a shared input generation technique to reduce computational load of input generation by amortizing costs across many models. Furthermore, we propose partitioning, pipelining, and RPC (Remote Procedure Call) coalescing software techniques to optimize embedding operations. To maintain efficiency at scale, we describe novel preemption notice and training hold mechanisms that minimize resource wastage, and ensure prompt error resolution. These techniques have demonstrated significant improvement in Google production, achieving a 116% performance boost and an 18% reduction in training costs across representative models.

==> requirements.tex <==
\section{Training System Requirements}
\label{sec:training_system_requirements}

From a system perspective, there are several properties desirable for a training framework for Ads recommendation and auction scoring models.

\subsection{Scalability, Performance/\$ and Efficiency}

Ads models typically train on petabytes of historical input data, across billions of events (i.e., training examples). Minimizing training time is important to developer velocity since it informs future experiments. We require models to train across many TPU chips, typically 64-256, while maintaining good scaling efficiency.

With a large number of models from several different teams training simultaneously, minimizing cost is of paramount importance. This includes choosing the right hardware that provides the best performance/\$, and implementing software optimizations that make executing the compute operations as efficient as possible. Minimizing other training overheads is of critical importance. These include: (1) generating and compiling the TensorFlow graph, (2) checkpointing, (3) input feature transformation, and (4) system interruptions. The end-to-end training system must spend the vast majority of time executing the ML compute operations that train the model, and minimize other overheads.

\subsection{Hardware Fungibility}

Due to the emergence of various types of hardware accelerators, it is imperative that our training infrastructure supports a variety of hardware types. Before we started adopting TPUs, our models were using CPU for training. Certain models with small amounts of floating point compute still use CPUs. Ensuring that models can execute on different hardware without requiring changes to them is of paramount importance. The user expresses only the semantics of the computation, and the training infrastructure builds different programs to orchestrate and optimize execution on different hardware. For most operations, this is accomplished by TensorFlow, but certain operations, like embeddings, are explicitly specialized by our infrastructure. All TPU generations training our production models are fungible, but the TPU embedding API and partitioning methodology are different from that on CPUs. Our infrastructure ensures that the differences in APIs are kept hidden from users.

\subsection{Initial vs Caught-Up Training}

Model training is organized into two distinct phases: (a) initial training on historical training data and (b) caught-up training on data as it streams in. We use the term advancing rate to refer to the number of events trained per unit of training time. If a model trains on a year’s worth of events in 2 days, the advancing rate is 365/2 or 184.5x. During initial training, models train on data collected over 2-3 years. The advancing rate must be 100x–500x for the model to train in a few days. We use a large number of TPU chips (64–256 chips) to sustain the high advancing rate. 

Once a model completes initial training, it is considered caught-up since it has trained on all events until the present, and the model transitions to caught-up training. During this phase, the model trains on newly arriving data. The advancing rate only needs to be 1x for the model to stay caught-up since training needs to be done only on the most recent data. We can use a small number of TPU chips (1–4 chips) to maintain the 1x advancing rate.

